Decision Making with Argumentation Graphs

This work is about making decisions by digital means. Funds should be distributed by the students of Heinrich-Heine-University. The proposals were made by the students themselves without further influence. For this purpose, dialog-based argumentation is used to give the participants a better understanding of various arguments. In addition, a software service has been developed which allows the students to express their preferences for various proposals. An experiment was carried out at the university, which should prove whether students are satisfied with this type of participation. The results indicate that the procedure is well accepted and thus successful. However, improvements to the process itself were necessary during the experiment and should be considered for future procedures. Further procedures are desired.

==> cd.tex <==
\chapter*{}
\thispagestyle{empty}

\begin{center}
  \vspace{-3cm}
  \fbox{\parbox[c][12cm][c]{12cm}{\centering Hier die Hülle\\[1cm]mit der CD/DVD einkleben}}
\end{center}

\vfill

\textbf{Diese CD enthält:}
\begin{itemize}
 \item eine \emph{pdf}-Version der vorliegenden \thesistype{}
 \item die \LaTeX- und Grafik-Quelldateien der vorliegenden \thesistype{} samt aller verwendeten Skripte
 \item \textbf{[anpassen]} die Quelldateien der im Rahmen der \thesistype{} erstellten Software XYZ
 \item \textbf{[anpassen]} den zur Auswertung verwendeten Datensatz
 \item die Websites der verwendeten Internetquellen
\end{itemize}

